Higher-Order Specifications for Deductive Synthesis of Programs with Pointers (Extended Version)

Synthetic Separation Logic (SSL) is a formalism that powers SuSLik, the state-of-the-art approach for the deductive synthesis of provably-correct programs in C-like languages that manipulate Heap-based linked data structures. Despite its expressivity, SSL suffers from two shortcomings that hinder its utility. First, its main specification component, inductive predicates, only admits first-order definitions of data structure shapes, which leads to the proliferation of ''boiler-plate'' predicates for specifying common patterns. Second, SSL requires concrete definitions of data structures to synthesise programs that manipulate them, which results in the need to change a specification for a synthesis task every time changes are introduced into the layout of the involved structures. We propose to significantly lift the level of abstraction used in writing Separation Logic specifications for synthesis -- both simplifying the approach and making the specifications more usable and easy to read and follow. We avoid the need to repetitively re-state low-level representation details throughout the specifications -- allowing the reuse of different implementations of the same data structure by abstracting away the details of a specific layout used in memory. Our novel high-level front-end language called Pika significantly improves the expressiveness of SuSLik. We implemented a layout-agnostic synthesiser from Pika to SuSLik enabling push-button synthesis of C programs with in-place memory updates, along with the accompanying full proofs that they meet Separation Logic-style specifications, from high-level specifications that resemble ordinary functional programs. Our experiments show that our tool can produce C code that is comparable in its performance characteristics and is sometimes faster than Haskell.

==> Makefile <==
MAIN=main
MAIN_EXTENDED=main

EXTENDED=#'\let\EXTENDED=1 \input'

EXTENDED_OUT=-jobname=extended 

all: $(MAIN).pdf 

# extended.pdf submission/final.tex

# NOTE: We use EXTENDED everywhere except the last execution of pdflatex
# so that we keep the appendix references
# main.pdf: $(MAIN).tex $(wildcard *.tex) *.bib
# 	pdflatex $(EXTENDED) $<
# 	bibtex $(patsubst %.tex,%.aux, $<)
# 	pdflatex $(EXTENDED) $<
# 	pdflatex $(MAIN).tex

main.pdf: $(MAIN).tex $(wildcard *.tex) *.bib
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main

extended.pdf: $(MAIN_EXTENDED).tex $(wildcard *.tex) *.bib
	pdflatex $(EXTENDED_OUT) $(EXTENDED) $(MAIN_EXTENDED).tex
	bibtex $(patsubst %.tex,%.aux, $<)
	pdflatex $(EXTENDED_OUT) $(EXTENDED) $(MAIN_EXTENDED).tex
	pdflatex $(EXTENDED_OUT) $(EXTENDED) $(MAIN_EXTENDED).tex

submission/final.tex: $(MAIN).tex $(wildcard *.tex) *.bib
	arlatex --outfile=submission/final.tex --document=$(MAIN).tex $(wildcard *.tex) *.bib

.PHONY: clean

clean:
	rm -f $(MAIN).aux
	rm -f $(MAIN).bbl
	rm -f $(MAIN).blg
	rm -f $(MAIN).out
	rm -f $(MAIN).log
	rm -f $(MAIN).pdf
	rm -f extended.aux
	rm -f extended.bbl
	rm -f extended.blg
	rm -f extended.out
	rm -f extended.log
	rm -f extended.pdf



==> case-studies.tex <==
% !TEX root = main.tex

\section{Case Studies}

\begin{center}
  \begin{table}[H]
  \begin{tabular}{ c c }
    \hline
    Symbol & Meaning \\
    \hline
    \works & Works\\
    \doesNotWork & Does not work\\
    \question & Synthesizes incorrectly\\
    \higherOrder & Requires higher-order functions for full implementation\\
    \hline
  \end{tabular}
    \caption{Legend}
  \end{table}
\end{center}

\begin{center}
  \begin{table}[H]
  \begin{tabular}{ c c }
    \hline
    Name & Status \\
    \hline
    \verb|cons| & \works\\
    \verb|car| & \question\\
    \verb|singleton| & \works\\
    \verb|fold| & \works \higherOrder\\
    \verb|map| & \works \higherOrder\\
    \verb|filterLt9| & \works\\
    \verb|snoc| & \works\\
    \verb|reverse| & \doesNotWork\\
    \verb|append| & \works \question\\
    \verb|zip| & \doesNotWork\\
    \verb|zipWith| & \works \higherOrder\\
    \verb|maximum| & \works\\
    \verb|scanr| & \doesNotWork \higherOrder\\
    \verb|selfAppend| & \doesNotWork\\
    \verb|take| & \doesNotWork\\
    \verb|replicate| & \doesNotWork\\
    \verb|foldMap| & \doesNotWork \higherOrder\\
    % \verb|subseqs| & \doesNotWork\\
    \verb|mapSum| & \works\\
    \verb|leftList| & \works\\
    \verb|sum| & \works\\
    \hline
  \end{tabular}
    \caption{Example Status}
  \end{table}
\end{center}




==> compile-latex-final.tex <==
  \input{main.tex}


==> compile-latex.tex <==



==> conclusion.tex <==
\section{Conclusion}


==> introduction.tex <==
% !TEX root = main.tex

\section{Introduction}

% [(DY): A couple of ideas to possibly identify as key concepts: (a) ``Layout polymorphism''. (b) Inductive predicates are closely related to two functional
% concepts: (1) \textit{algebraic datatypes} (2) \textit{pattern matching FP-style functions}. Both of these are represented by our translation using
% inductive predicates.]

%Separation logic has seen success in both verifying properties of pointer-manipulating code and in program synthesis tools such as \suslik~\cite{ohearn:2001:seplogic,polikarpova:2019:suslik,reynolds:2002:seplogic}.
% We propose to significantly lift the level of abstraction used in writing specifications. By moving away from the need to repetitively express low-level data structure details throughout the specification, we aim to 

%However, as the level of abstraction is typically low, more complex
%separation logic specifications can be verbose and difficult to read.
%Furthermore, the low-level representation of data structures must be
%used directly throughout the specification. This means that
%specifications cannot be reused for different implementations of the
%same data structure if they have different layouts in memory.

%To address these two difficulties, we develop a high-level front-end
%language, for the program synthesis tool \suslik called
%\tool.\footnote{ Pikas might look similar to susliks, but are more nimble and have a longer life expectancy. }
%
%\suslik is based on a variant of separation logic called
%\textit{synthetic separation logic} or
%SSL~\cite{polikarpova:2019:suslik}.

Recent advances in program synthesis allow programmers to concentrate
on stating precise specifications --- leaving the job of generating
provably correct and efficient code to the synthesiser, such
as~\suslik~\cite{ohearn:2001:seplogic,polikarpova:2019:suslik,reynolds:2002:seplogic}.
Such specifications are usually expressed using (Synthetic) Separation
Logic that while hugely successful in verifying properties of
pointer-manipulating programs remains out of reach to many mainstream
developers. As the programs grow in complexity, such SSL
specifications can become exceedingly verbose and complex --- making
the job of specification writer especially error-prone and defeating
the purpose of a \textit{usable proof automation toolchain}.

We propose to significantly lift the level of abstraction used in
writing separation logic specifications ---both simplifying the
approach and making the specifications more usable and easy to read
and follow. We avoid the need to repetitively re-state low-level
representation details throughout the specifications --- allowing the
reuse of different implementations of the same data structure by
abstracting away the details of a specific layout used in memory. Our
novel \textit{high-level front-end language}
called~\tool~\footnote{Pikas might look similar to susliks, but are
  more nimble and have a longer life expectancy.} takes \suslik to the
next level of expressivity and simplicity. \tool has a syntax similar
to functional programming languages, based on algebraic data types
(ADTs).

In addition to being more succinct,
\tool also addresses the reusability issue. By manipulating ADTs, the
functions do not need to deal with the specific memory layouts of the
data structures. This separates the code that operates on data
structures from the low-level details of the implementations of the
data structures. Our contributions are as follows:

%We make the following contributions:

\begin{itemize}
  \item A high-level front-end language to synthetic separation logic
  \item An extension to \suslik's specification language to enable this high-level language
    to be implemented (Section~\ref{sec:extensions})
  \item Memory layout-agnostic synthesis from a functional specification
  \item A performance and expressiveness evaluation of the \tool tool (Section~\ref{sec:evaluation})
\end{itemize}


% Synthetic separation logic, or SSL, is a specification language that has seen some success in the field of program
% synthesis.
% However, the level of abstraction has largely remained relatively low. Specifications are expressed in terms of
% direct pointer manipulations. The primary mechanism of abstraction is the \textit{inductive predicate}. While
% this allows the programmer to describe a variety of data structures, including linked lists and trees, it does
% so at the level of pointers.
%
% In this paper, we examine a new form of abstraction for SSL-based synthesis tools. We focus specifically on the
% \suslik SSL-based synthesis tool. % TODO: \suslik citations
%
% We develop
% a higher-level programming language \tool which compiles down to a \suslik specification. This language shares
% many characteristics with functional programming languages in the style of Haskell. It includes features
% such as algebraic data types, pattern matching and Boolean guards. The design of this language is based on the following three key ideas:
% \\
%
% \tbox{
% \textbf{Three key ideas}:
% \begin{enumerate}
%   \item Algebraic data types (ADTs) can be represented as inductive predicates.
%
%   \item Recursive functions on ADTs that pattern match on their arguments can also be represented as inductive predicates.
%
%   \item The ``interface'' between the high-level abstraction of ADTs and the low-level implementation of them as inductive predicates can be expressed using a language construct called a ``layout.''
%
%   % \item The \lstinline{layout} language construct in the high-level \fnLang language. This feature
%   % allows the programmer to express inductive predicate representations of an ADT.
% \end{enumerate}
% }
% \\
%
% To justify the language semantics, in Section~\ref{sec:formal} we write a formal semantics for the translation and show that it is sound relative
% to a standard intepretation for \fnLang. We use the following plan to accomplish this goal.
% \\
%
% \tbox{
% \textbf{The Soundness Plan}:\\
%   \begin{itemize}
%     \item We define an abstract machine semantics for a representative subset of \fnLang.
%     \item We give a formal definition of the translation of that subset of \tool into SSL.
%     \item We prove the following soundness theorem. For any well-typed \tool expression $e$, the SSL translation of $e$ is satisfied
%       by the ending state of the store and heap given by reducing the expression using the abstract machine semantics. This is Theorem~\ref{thm:gen-soundness} in Section~\ref{sec:soundness}.
%     % \item We prove the soundness theorem: \textit{Subject to a few conditions such as well-typedness, any terminal state of the abstract machine when given a \tool function application is a model for the SSL proposition given by the translation of that function application}.\\
%   \end{itemize}
% }
% \\
%
% \noindent
% The specifics of this are given in Section~\ref{sec:formal}.
%

